GAQAT: gradient-adaptive quantization-aware training for domain generalization

Research on loss surface geometry, such as Sharpness-Aware Minimization (SAM), shows that flatter minima improve generalization. Recent studies further reveal that flatter minima can also reduce the domain generalization (DG) gap. However, existing flatness-based DG techniques predominantly operate within a full-precision training process, which is impractical for deployment on resource-constrained edge devices that typically rely on lower bit-width representations (e.g., 4 bits, 3 bits). Consequently, low-precision quantization-aware training is critical for optimizing these techniques in real-world applications. In this paper, we observe a significant degradation in performance when applying state-of-the-art DG-SAM methods to quantized models, suggesting that current approaches fail to preserve generalizability during the low-precision training process. To address this limitation, we propose a novel Gradient-Adaptive Quantization-Aware Training (GAQAT) framework for DG. Our approach begins by identifying the scale-gradient conflict problem in low-precision quantization, where the task loss and smoothness loss induce conflicting gradients for the scaling factors of quantizers, with certain layers exhibiting opposing gradient directions. This conflict renders the optimization of quantized weights highly unstable. To mitigate this, we further introduce a mechanism to quantify gradient inconsistencies and selectively freeze the gradients of scaling factors, thereby stabilizing the training process and enhancing out-of-domain generalization. Extensive experiments validate the effectiveness of the proposed GAQAT framework. On PACS, our 3-bit and 4-bit models outperform direct DG-QAT integration by up to 4.5%. On DomainNet, the 4-bit model achieves near-lossless performance compared to full precision, with improvements of 1.39% (4-bit) and 1.06% (3-bit) over the SOTA QAT baseline.

==> archive.tex <==
\section{Preliminary}
\label{gen_inst}

\subsection{Quantization}
Uniform quantization is favored in neural networks for its hardware efficiency. 
The range of full-precision value $x$ is divided into equal intervals, and each interval is assigned a quantization level.
% Each layer employs two distinct scaling factors to accommodate varying distributions of weights and activations, facilitating efficient inference. This approach converts full-precision activations and weights into low-precision integers.
% In \(b\)-bit quantization, activations are limited to the range \([0, 2^b - 1]\) and weights to \([-2^{b-1}, 2^{b-1} - 1]\). 

The uniform quantization function is defined as:
\(
\hat{x} = Q_b(x; s) = s \times \left\lfloor \text{clip}\left( \frac{x}{s}, l, u \right) \right\rceil,
\)
where $\hat{x}$ is the de-quantized value, \(\lfloor \cdot \rceil\) denotes round-to-nearest operator, \(s\) is a learnable scaling factor in QAT, and the \(\texttt{clip}\) function ensures values stay within the bounds \([l, u]\). Specifically, in \(b\)-bit quantization, for activation quantization, we set \(l = 0\) and \(u = 2^b - 1\); for weight quantization, we set \(l = -2^{b-1}\) and \(u = 2^{b-1} - 1\).

Due to the non-differentiability of the rounding operation, the Straight-Through Estimator (STE) \yym{add cite} is employed to approximate the gradients.
% , ensuring smooth training. 
The gradient approximation is given by:
\(
\frac{\partial L}{\partial x} \approx \frac{\partial L}{\partial \hat{x}} \cdot 1_{l \leq \frac{x}{s} \leq u},
\)
where \(1_A\) is an indicator function that is 1 if the element is within set \(A\) and 0 otherwise.
\subsection{DOMAIN GENERALIZATION}

This paper explores the domain generalization task within the scope of classification tasks.
We denote the input as \( \mathbf{x} \in \mathbb{R}^d \) and the label as \( y \in \{1, \ldots, C\} \). 
For a typical domain generalization problem, we can access $E$ source domains $\mathcal{S}=\{D_e=(\mathbf{x}_i^e, y_i^e)_{i=1}^{n_e}\}_{e=1}^E$  in the training stage, where $D_e$ is the sampled dataset for domain \( e \) and $n_e$ is the sample size.

% In a classification problem,
% % Each domain \( e \) has its specific data distribution \( Q_e \).
% % but they share the same set of classes.
% The sampled dataset for domain \( e \) is \( D_e = \{(x_i, y_i)\}_{i=1}^{n_e}, \) where \( (x_i, y_i) \sim Q_e \) and $Q_e$
% is the probability distribution of domain $e$.
% The model parameters are \( \theta \in \mathcal{O}, \) where \( \mathcal{O} \) is the set of parameters. 
Given the dataset \( D_e \), the loss function is defined as \( L_{D_e}(\theta) = \frac{1}{n_e} \sum_{i=1}^{n_e} L(f_\theta(x_i), y_i). \)

The training objective is to minimize the overall risk \( L(\theta) \) across all domains, but in practice, we can only access the source domain dataset \( D_s, \) whose distribution is \( Q_s. \) Since \( Q_s \) differs from the true distribution \( Q, \) the model parameters trained only on the source domain data \( \theta_s = \arg \min_\theta L_{D_s}(\theta) \) may not achieve optimal performance in unseen domains. Therefore, the key to domain generalization is to optimize the parameters using the source domain data \( D_s \) to improve the model's generalization ability in unseen domains. 

Sharpness-Aware Minimization (SAM) (Foret et al., 2020) is a foundational method that seeks the flat minimum of the loss function \( L(\theta) \) . It helps enhance generalization across domains by minimizing the perturbed loss, where \( \hat{\epsilon} \) is a perturbation vector and \( \rho \) controls the perturbation size:\(\min_\theta L(\theta + \hat{\epsilon}; D), \quad \hat{\epsilon} = \rho \frac{\nabla L(\theta; D)}{\|\nabla L(\theta; D)\|}\).

SAGM extends SAM by focusing three objectives: empirical risk \( L(\theta; D) \), perturbed loss \( L_p(\theta; D) \), and the surrogate gap \( h(\theta) \): \( \min \big(L(\theta; D), L_p(\theta; D), h(\theta)\big) \). Minimizing \( L(\theta; D) \) and \( L_p(\theta; D) \) finds low-loss regions, while minimizing \( h(\theta) \) ensures a flat minimum. This combination improves both training performance and generalization. The overall optimization is:\(\min L(\theta; D) + L_p(\theta - \alpha \nabla L(\theta; D); D)\)
where \( \alpha \) is a hyperparameter. This can be rewritten as:
\(
\min L(\theta; D) + L(\theta + \hat{\epsilon} - \alpha \nabla L(\theta; D); D)
\)
with \( \hat{\epsilon} = \rho \frac{\nabla L(\theta; D)}{\|\nabla L(\theta; D)\|} \).

\subsection{Quantization in DOMAIN GENERALIZATION}
% 由于此前没有工作探索过DG场景下的量化流程，所以我们在这里定义我们的流程，如图x, 我们会先有一个已经预训练好的，有一定泛化性能的模型\theta_0, 然后在QAT的过程中，我们只能使用the source domain data \( D_s \)，可以有一个或者多个，然后受到sam及其变体的启发，我们也对量化目标引入了平滑因子，以求获得更好的泛化性能，最后我们通过源数据和现有的优化目标进行QAT训练，获得泛化性能良好的量化模型，其中泛化性在目标域\( D_d \)上进行测试。the loss function is defined as \(\min L(Q(\theta); D) + L_p(Q(\theta - \alpha \nabla L(Q(\theta); D); D))\)
Given the lack of prior research on quantization processes in Domain Generalization (DG) scenarios, we establish our approach, illustrated in Figure \ref{fig:process}. We start with a pre-trained model, \( \theta_0 \), which possesses initial generalization capabilities. During QAT, we exclusively utilize source domain data \( D_s \), which may encompass one or more datasets. SAM and its variants, we incorporate a smoothing factor into our quantization objective to enhance generalization. We then proceed with QAT, employing source data and our defined optimization objectives, to develop a quantized model verified for generalization in the target domain \( D_d \). The loss function is defined as: 
\begin{equation}
    \min L(Q(\theta, s_w); Q(D, s_a)) + L_p(Q(\theta - \alpha \nabla L(Q(\theta, s_w); Q(D, s_a)), s); Q(D, s_a))
    \label{eq:sagm_qat}
\end{equation}
In the quantization process, the unique scale factor is closely linked to the distribution of weights and activations during actual operations, compared to full-precision targets. After introducing a flatness objective, a significant change is that the scale factor will correspond to two targets, thus producing two sets of gradients. One set is the original accuracy-related gradient, which we abbreviate as \( g_{\text{scale}_{\text{acc}}} \), and the other is the newly introduced flatness-related gradient, abbreviated as \( g_{\text{scale}_{\text{smo}}} \). We anticipate that this dual-gradient strategy will help optimize both the generalization performance and accuracy of the model. However, we have found that directly adopting this objective can lead to performance degradation, as the two target gradients associated with the same scale factor may significantly interfere with each other, thereby impairing overall performance. Our research focuses on introducing a training method aimed at reducing this interference to enhance model quantization performance in DG scenarios. (???? 需要放干扰的图吗)




% Let the input \( x \in \mathbb{R}^d \) and the label \( y \in \{1, \ldots, C\} \). Each domain \( e \) has its specific data distribution \( Q_e \), but they share the same set of classes. The dataset for domain \( e \) is \( D_e = \{(x_i, y_i)\}_{i=1}^{n_e}, \) where \( (x_i, y_i) \sim Q_e. \) The model parameters are \( \theta \in \mathcal{O}, \) where \( \mathcal{O} \) is the set of parameters. Given the dataset \( D_e \), the loss function is defined as 
% 为从一个已有的训练好有一定泛化性能的全精度模型开始，进行source数据域的QAT量化训练，最后获得量化好的模型，在traget域上进行测试来获得test acc.,(这段用公式来表示)，如图所示（缺对比流程图，对比dg场景和iid场景下量化的区别）
% 受到sagm的启发，我们也认为引入平坦因子的考虑可能导向更好的dg性能，所以我们的优化目标从xx 变成了xx. 但相比全精度而言，量化里面的缩放因子对模型运算时的真实权重和激活影响重大，他们会直接影响权重和激活的分布，所以本文重点关注的是量化独有的scale的梯度部分，即acc scale和 smooth scale（用公式表达出来）

% 全精度下的dg基本定义和目标
% 讲讲dg的基本公式和目标，然后讲讲sagm变体的目标
% 然后讲我们对于dg下量化的首次定义，并且给出公式和关注重点

% 在多类分类任务中，设 \( x \in \mathbb{R} \) 为输入，\( y \in \{1, ..., k\} \) 为相应的类别标签。每个领域 \( e \) 都有其特定的数据分布 \( Q_e \)。例如，自动驾驶汽车在白天和夜间采集的数据可视为两个不同的领域。领域 \( e \) 的数据集记为 \( D_e = \{(x_i, y_i)\}_{i=1}^{n_e} \)，其中 \( (x_i, y_i) \sim Q_e \)，且 \( n_e \) 是领域 \( e \) 中的数据样本数量。

% 给定模型参数 \( \theta \)，定义领域 \( e \) 的损失函数为 \( C_D(\theta) \)，表示领域的总体风险。训练的目标是在所有领域中最小化总体风险，但在实际中，我们只能获取源域的数据 \( D_s \)。由于源域分布 \( Q_s \) 与真实分布 \( Q \) 之间存在差异，仅基于源域数据训练的模型可能无法很好地泛化到未见领域。因此，领域泛化的目标是通过源域数据 \( D_s \) 优化参数 \( \theta^* = \arg \min L(\theta) \)。

% 最近，随着对参数空间进行优化的研究兴起（Foret 等人，2020；Kwon 等人，2021），多个研究针对模型参数 \( \theta \) 过拟合于训练数据集的问题进行了研究（Wang 等人，2023；Zhang 等人，2023）。这些研究表明，在扰动的参数区域进行优化可以提升模型的泛化能力。为了构建能够适应未知领域的模型，必须确保优化后的参数不会过拟合于源域数据。因此，参数扰动作为避免过拟合的一种方法得到了探索。

% 在各种方法中，Sharpness-Aware Minimization (SAM)（Foret 等人，2020）是最基础的参数扰动方法之一。它通过优化以下公式来使 \( \theta \) 的局部区域趋于平坦的最小值：

% \[
% \min_{\theta} \max_{\epsilon} L(\theta + \epsilon)
% \]

% 其中，\( \epsilon \) 是扰动向量，\( \rho \) 表示最大扰动大小。该方法有助于提高模型在不同领域的泛化能力。



% 在本文中，我们假设神经网络 \( f \) 在多个源域 \( D = \{D_1, ..., D_s\} \) 上进行训练，且存在一个目标域 \( T \)。对于每个源域 \( D_i \)，训练数据由样本 \( \{(x_j^i, y_j^i)\}_{j=1}^{n_i} \sim D_i \) 组成。所有源域的训练损失定义为：

% \[
% L(\theta; D) = \frac{1}{Sn} \sum_{i=1}^{s} \sum_{j=1}^{n_i} \text{交叉熵}(f(x_j; \theta), y_j^i)
% \]

% 这对应于一个经验风险最小化（ERM）问题。为了提高泛化能力，引入了 SAM 方法，该方法通过在局部邻域内寻找最坏情况下的损失最小化参数：

% \[
% \min_\theta \max_{\epsilon \leq \rho} L(\theta + \epsilon; D)
% \]

% 通过对 \( \theta \) 进行泰勒展开，内层的最大化问题可以近似为：

% \[
% \epsilon \approx \rho \frac{\nabla L(\theta; D)}{||\nabla L(\theta; D)||}
% \]

% 因此，SAM 优化问题简化为：

% \[
% \min_\theta L(\theta + \hat{\epsilon}; D), \quad \hat{\epsilon} = \rho \frac{\nabla L(\theta; D)}{||\nabla L(\theta; D)||}
% \]

% 换句话说，SAM 通过最小化扰动损失 \( C_p(\theta; D) = L(\theta + \hat{\epsilon}; D) \) 来确保模型不仅在原始损失曲面上进行优化，还能更好地泛化。

% 受此前分析的启发，满足以下条件有助于实现良好的泛化性能：(i) 首先，目标最小值附近的损失应该足够低；(ii) 其次，找到的最小值应位于平坦的损失曲面上。为满足这两个条件，我们提出了SAGM方法，用以同时最小化三个目标：经验风险损失 \( L(\theta; D) \)、扰动损失 \( C_p(\theta; D) \) 和替代间隙 \( h(\theta) \)：

% \[
% \min (L(\theta; D), C_p(\theta; D), h(\theta))
% \]

% 直观上，我们通过最小化 \( L(\theta; D) \) 和 \( C_p(\theta; D) \) 来搜索低损失区域，同时通过最小化 \( h(\theta) \) 来寻找平坦的局部最小值。较低的损失意味着较小的训练误差，代表模型在源训练数据上的良好表现，而平坦的损失曲面则有助于减少训练和测试表现之间的泛化差距。当两个目标同时满足时，训练出的模型预期将具有较高的预测准确性和良好的泛化能力。

% 为实现这一目标，我们设计了如下优化目标：

% \[
% \min (L(\theta; D) + C_p(\theta - \alpha \nabla L(\theta; D); D))
% \]

% 其中 \( \alpha \) 是一个超参数。我们可以将其重写为：

% \[
% \min L(\theta; D) + L(\theta + \hat{\epsilon} - \alpha \nabla L(\theta; D); D)
% \]

% 其中 \( \hat{\epsilon} \leq \rho \frac{\nabla L(\theta; D)}{||\nabla L(\theta; D)||} \)（更多细节请参考第3节中的方程3）。因此，优化问题变为：

% \[
% \min L(\theta; D) + L(\theta + (\frac{\rho}{||\nabla L(\theta, D)||} - \alpha) \nabla L(\theta; D); D)
% \]

% 从方程13可以看出，我们的方法只需要计算损失 \( L(\theta; D) \) 和 \( L(\theta + (\frac{\rho}{||\nabla L(\theta, D)||} - \alpha) \nabla L(\theta; D); D) \)。请注意，后者的计算成本与 \( L(\theta; D) \) 相同。考虑到在计算 \( \nabla L(\theta; D) \) 时已经计算了 \( L(\theta; D) \)，SAGM 的计算成本与 SAM 基本相同。
% 整合写到一起

% 由于此前没有工作探索过DG场景下的量化流程，所以我们在这里定义我们的流程为从一个已有的训练好有一定泛化性能的全精度模型开始，进行source数据域的QAT量化训练，最后获得量化好的模型，在traget域上进行测试来获得test acc.,(这段用公式来表示)，如图所示（缺对比流程图，对比dg场景和iid场景下量化的区别）
% 受到sagm的启发，我们也认为引入平坦因子的考虑可能导向更好的dg性能，所以我们的优化目标从xx 变成了xx. 但相比全精度而言，量化里面的缩放因子对模型运算时的真实权重和激活影响重大，他们会直接影响权重和激活的分布，所以本文重点关注的是量化独有的scale的梯度部分，即acc scale和 smooth scale（用公式表达出来）

\section{Method}
\label{others}
\subsection{Scale gradient conflict in DG scenario}
% 在量化中很重要的一个元素是可学习的缩放因子，在我们引入的DG场景下的公式当中，除了原始的g_{scale_{acc}}，还有一个g_{scale_{smooth}}，也就是说实际上每一个缩放因子会接受两个梯度，保证loss的低与平坦。为了说明两个梯度之间存在的冲突现象，我们在pacs上进行测试，将art域作为test域，其他三个作为训练域，每隔300step记录一次scale的这300step里面的梯度真实值的和，我们观测到两个梯度之间存在着显著的冲突，表现在反向以及一方会有异常值的突变，而论文Oscillation-free Quantization for Low-bit Vision Transformers中提到由量化的离散性质引起的权重振荡可以通过存在一个可学习的缩放因子而被极大地放大，所以我们认为这本身对于qat的性能而言，不论是iid还是ood,可能是一个极大的负面影响，并且从冲突的角度来说，反向的梯度之间互相会影响双方的收敛，从而不好平衡准确性scale和平坦性scale的收敛。如图x, 我们观察到，是随着训练的进行，在部分层会出现一个准确率scale和平滑scale的梯度反向并且接近平衡的一个状态，也就是说这些层的scale会进入一个收敛的状态, 但是很显然，就单个准确率scale或者平坦性scale而言，这些层都未收敛，也就是说在准确性和平坦性上，这些层的scale其实进行了一个平衡。
In the quantization process, a key element is the learnable scale factor. In our Domain Generalization (DG) scenario, besides the original accuracy-related gradient \(g_{\text{scale}_{\text{acc}}}\), we have also introduced a smoothness-related gradient \(g_{\text{scale}_{\text{smo}}}\). This means each scale factor actually receives two gradients to ensure both low loss and smoothness. However, in our tests on the PACS dataset, with the art domain as the test domain and the other three as training domains, we record the cumulative gradients for the scale factor every 300 steps. As shown in Figure \ref{fig:conflict}

\begin{figure}[htbp]
    \centering
    % First image
    \begin{minipage}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{conflict.png}
        \caption{Enter Caption for the first image}
        \label{fig:conflict}
    \end{minipage}
    \hfill % Adds horizontal space between the two images
    % Second image
    \begin{minipage}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{opposite.png}
        \caption{Enter Caption for the second image}
        \label{fig:opposite}
    \end{minipage}
\end{figure}
, we observe significant conflicts between the two gradients, manifesting as opposing gradients or sudden anomalies.

According to the paper "Oscillation-free Quantization for Low-bit Vision Transformers," the weight oscillations caused by the discrete nature of quantization can be significantly amplified by a learnable scale factor. Thus, we believe this phenomenon could have a substantial negative impact on the performance of QAT, whether in IID or DG scenarios. From the perspective of gradient conflict, interacting gradients may affect each other's convergence, making it challenging to balance the scales for accuracy and smoothness simultaneously.

As depicted in Figure \ref{fig:opposite}, during training, we notice that in certain layers, the accuracy-related and smoothness-related scale gradients are opposite and tend to balance each other, suggesting that these layers' scale factors are reaching a state of convergence. However, it is apparent that for individual accuracy or smoothness scales, these layers have not truly converged but are instead balancing between accuracy and smoothness.

Although SAGM successfully resolves conflicts between \( w \) and \( w_p \) by optimizing the angle between them in full-precision targets, our scale gradients only have positive and negative directions, so we cannot use an angle approximation method to resolve these conflicts.



%以往的梯度冲突解决方案，解释为什么不行，我们的情况是什么样解释，会有突变的梯度，会有些层收敛到反向均衡状态，放图，直接用一个的梯度区别（），直接用一个会丢失性能，用两个会有冲突，所以启发我们选择性丢弃一些
% 对二者收敛都不好
% OB1 3.1 准确率scale和平滑scale的平衡性
% While training is possible, there still many challenges exist in weight-sharing in practice. For example, ABN [48] observes a large accuracy gap between the lower bit-widths and higher bit-widths. These works simply bypass this problem and remove the ultra-low bit-width until the training becomes stable, however, doing so does not achieve high compression ratios.
% To illustrate the bit-width interference in weight-sharing quantization, we use a 2D regression quantization experiment depicted in Fig. 1. Our optimization objective minimizes the empirical risk [8, 35]:



% In the quantization process, the learnable scaling factor is a critical element. In the Domain Generalization (DG) scenario we propose \ref{eq:sagm_qat}, in addition to the original accuracy-related learning factor, we introduce a smoothness-related learning factor. In other words, each learning factor receives two gradients simultaneously, which are used to reduce the loss and maintain the smoothness of the loss.

% During our experiments on the PACS dataset, we used the art domain as the test domain, while the other three domains were used for training. We recorded the gradient sum of the scaling factor every 300 steps, and the results showed significant interference between the two gradients, manifested as gradient reversals and abrupt outlier values.

% The mutual interference between the gradients affects the balance between accuracy and smoothness, potentially leading to suboptimal convergence for both. Additionally, the paper Oscillation-free Quantization for Low-bit Vision Transformers points out that due to the discrete nature of quantization, weight oscillations can be significantly amplified by the learnable scaling factor. Based on this, we believe that this interference negatively impacts the performance of Quantization-Aware Training (QAT).
%在量化中很重要的一个元素是可学习的缩放因子，在我们引入的DG场景下的公式当中，除了原始的准确率学习因子，还有一个平滑性学习因子，也就是说实际上每一个学习因子会接受两个梯度，保证同时兼顾loss低和loss平坦。但是我们在pacs上进行测试，将art域作为test域，其他三个作为训练域，每隔300step记录一次scale的这300step里面的梯度真实值的和，我们观测到两个梯度之间存在着显著的干扰，表现在反向以及一方会有异常值的突变，而论文Oscillation-free Quantization for Low-bit Vision Transformers中提到由量化的离散性质引起的权重振荡可以通过存在一个可学习的缩放因子而被极大地放大，所以我们认为这本身对于qat的性能而言，不论是iid还是ood,可能是一个极大的负面影响，并且从干扰的角度来说，反向的梯度之间互相会影响双方的收敛，从而不好平衡准确性scale和平坦性scale的收敛。
\begin{figure}[htbp]
    \centering
    % Define the width of each subfigure to fill the line, with slight adjustments for spacing
    \begin{subfigure}[b]{0.32\linewidth}  % Adjust the width to use slightly less than one-third of the line
        \centering
        \includegraphics[width=\linewidth]{distort.png}  % Use the entire width of the subfigure
        \caption{Caption for image (a)}
        \label{fig:distort}
    \end{subfigure}
    \hfill  % Fills the space between the subfigures
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{distort2.png}
        \caption{Caption for image (b)}
        \label{fig:distort2}
    \end{subfigure}
    \hfill  % Ensures the figures are evenly spaced
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{distort3.png}
        \caption{Caption for image (c)}
        \label{fig:distort3}
    \end{subfigure}
    \caption{General caption for all three images.}  % Caption for the entire figure
\end{figure}


\subsection{混乱度Selective freezing to resolve gradient conflicts.}
% 为了解决上述的scale梯度冲突问题，我们提出了选择性冻结scale梯度策略，
% 首先为了清晰起见，我们定义梯度混乱度如下
% % Definition 3.1梯度混乱度
% 假设有K个step, 每个step存在一个梯度g_i, 那么第一个梯度集合记为S1 = {g_1, g_2, ..., g_{K-1}}, 第二个梯度集合就是S2 = {g_2, g_3, ..., g_K}, 记sgn为符号函数，则混乱度为 num(sgn(S1) != sgn(S2)) / K, 即K个step中与前一个step梯度相反方向的比例
% 由于混乱度可以判断一段训练过程中梯度的方向性，假如混乱度越低，说明训练的方向一致，梯度的正确性得到一定保证，注意，这里的逻辑并不能说明混乱度越高，就梯度的正确性没有保证，而且混乱度低能保证一定的正确性，为了观测准确率scale和平坦性scale的梯度混乱度特性，我们采用pacs数据集的0域进行test, 其他域用作train, 在4bit，下采用K=300, 约6个ep的数据，进行了观测，如图x所示，可以发现有部分层是有着准确率scale梯度混乱度随着训练进行而显著下降的现象的，也就是随着训练的进行，部分层的准确率scale梯度方向性越发一致，这似乎有点反直觉，而平坦度scale的梯度混乱度则在各个层中无显著的变化趋势，这个现象在3bit以及domainnet数据集上也有观测到，是一个共性现象。这启发我们，训练过程中准确率scale梯度可能会影响smooth scale梯度的训练，受到rsc以及freeze的启发，我们可以丢弃部分acc scale的训练梯度，来达到更好泛化性的目的。


% 此外，经过统计，我们发现，在acc scale混乱度降低的层中，降低到一定比例会出现两个梯度反向平衡的状态，换句话说，反向平衡的层和acc scale混乱度降低的层具有相当大的重叠，我们假设冻结混乱度低的acc scale，可以增强smooth scale的学习，对此，我们采取了一个简单的实验，如图x所示，这表示同一个scale在冻结准确率scale和未冻结两种情况下的真实梯度和情况，图x2表示在冻结了图1的准确率scale之后以及未冻结的情况下其余scale的梯度情况，可以发现被冻结的scale会开始继续训练，也就是平滑性会继续训练，而其他未冻结层的梯度波动程度显著减小，这说明梯度的波动不稳定性一定原因是scale之间训练不稳定干扰导致。这启发我们可以采取选择性冻结的方式来优化训练过程中的scale不稳定性以及平滑性收敛不足的问题。
% 但是假如在acc scale达到一定的混乱度时就冻结，持续冻结不解冻会导致训练的次优，所以我们采用每K步进行判断，如果混乱度低于阈值r, 则进行K步的冻结，否则取消冻结，每K步选择新的冻结区间

% 伪代码如下

% 为了解决上述scale梯度冲突问题，我们提出了一种选择性冻结scale梯度的策略。首先，为了清晰起见，我们定义梯度混乱度如下：

% **梯度混乱度（Definition 3.1）**  
% 假设有K个步长，每个步长对应一个梯度 \( g_i \)，那么第一个梯度集合记为 \( S1 = \{g_1, g_2, ..., g_{K-1}\} \)，第二个梯度集合记为 \( S2 = \{g_2, g_3, ..., g_K\} \)。记 \( sgn \) 为符号函数，则混乱度定义为：  
% \[
% \frac{num(sgn(S1) \neq sgn(S2))}{K}
% \]  
% 即在K个步长中，梯度方向与前一个步长相反的比例。

% 由于混乱度能够反映训练过程中梯度方向的一致性，混乱度越低表明训练方向较为统一，梯度的正确性在一定程度上得到了保证。需要注意的是，混乱度高并不一定意味着梯度的正确性受损，但混乱度低可以提供一定的正确性保障。

% 为了观察准确率scale和平滑性scale的梯度混乱度特性，我们在PACS数据集上以0域为测试集，其他域作为训练集，在4bit量化条件下，以K=300，约6个epoch的数据进行了实验。如图x所示，部分层的准确率scale梯度混乱度随着训练的进行显著下降，表明随着训练的进行，这些层的准确率scale梯度方向性变得更加一致，尽管这有些反直觉。而平滑性scale的梯度混乱度在各个层中没有明显的变化趋势。这一现象在3bit量化以及DomainNet数据集上也得到了验证，表现出一致性。

% 这一发现启发我们，准确率scale的梯度训练可能会影响平滑性scale的训练。受到RSC和freeze策略的启发，我们可以丢弃部分准确率scale的梯度，从而提高模型的泛化性能。



% 此外，经过统计，我们发现当准确率scale的混乱度降低到一定水平时，部分层的梯度会进入反向平衡状态。换句话说，反向平衡的层与混乱度降低的层有很大的重叠。
%Assumption 3.1 (不准确的scale收敛影响其他scale的训练).
% 从观测结果来看，部分 scale 能够达到准确率 scale（acc scale）与平滑性 scale（smooth scale）之间的反向平衡状态，并表现出收敛的迹象。然而，重要的是要认识到，这种表面上的收敛并不意味着 acc scale 或 smooth scale 已经达到了良好的收敛状态。进一步的观察发现，acc scale 的梯度混乱度逐渐降低的层与最终达到反向平衡收敛状态的层高度重合，这种不恰当的收敛可能会对平滑性 scale 的训练产生不利影响，并且这种次优的收敛不仅可能影响特定层的训练效果，还可能对其他层的训练产生影响，包括梯度异常值的出现。 

% 为了验证这一假设，我们进行了一项实验。我们将准确率 scale 的梯度混乱度作为判断收敛情况的指标。图 x 展示了在冻结与未冻结准确率 scale 的条件下，同一 scale 的真实梯度变化情况；图 x2 则展示了在冻结准确率 scale 后其他 scale 的梯度波动情况。实验结果表明，不仅冻结的 scale 能够继续进行平滑性训练，而且未冻结层的梯度波动却显著减少。这一发现强调了平滑性 scale 的梯度确实没有达到良好的收敛状态，且次优收敛scale和其他scale 之间的训练干扰会影响梯度的不稳定性。

% 由此我们推断，选择性冻结准确率scale的方式可以有效解决训练过程中的scale不稳定性问题，并改善平滑性收敛的不足。然而，持续冻结不解冻可能会导致训练结果次优，因此我们采用了一种动态策略：每K步判断一次混乱度，当混乱度低于阈值 \( r \) 时冻结该scale的K步训练，否则取消冻结。每K步重新选择新的冻结区间。
% 伪代码如下：

To address the issue of scale gradient conflict, we propose a selective freezing strategy for scale gradients. First, for clarity, we define gradient disorder as follows:

\textbf{(Definition 3.1) }  Gradient Disorder
Assume there are K steps, and each step corresponds to a gradient \( g_i \). The first gradient set is denoted as \( S1 = \{g_1, g_2, ..., g_{K-1}\} \), and the second gradient set as \( S2 = \{g_2, g_3, ..., g_K\} \). Let \( sgn \) be the sign function. The disorder is then defined as:  
\[
\frac{num(sgn(S1) \neq sgn(S2))}{K}
\]  
This represents the proportion of steps where the gradient direction is opposite to that of the previous step.

Since disorder reflects the consistency of gradient direction during training, lower disorder indicates more consistent training direction and implies a certain level of correctness in the gradients. It is important to note that high disorder does not necessarily mean incorrect gradients, but low disorder can guarantee a certain degree of correctness.

To observe the gradient disorder characteristics of accuracy scale and smoothness scale, we conducted experiments on the PACS dataset, using domain 0 as the test set and the other domains as the training set. Under 4-bit quantization, with K=300 and about 6 epochs of data, we observed the results. As shown in Figure \ref{fig:distort} and \ref{fig:distort2}, we found that in some layers(not all, such as \ref{fig:distort3}), the gradient disorder of the accuracy scale decreases significantly as training progresses, indicating that the gradient direction of the accuracy scale in these layers becomes increasingly consistent, despite this being somewhat counterintuitive. However, the gradient disorder of the smoothness scale showed no significant change across layers. This phenomenon was also observed under 3-bit quantization and on the DomainNet dataset, indicating it is a common occurrence.





This observation suggests that the gradient training of the accuracy scale may influence the training of the smoothness scale. Inspired by the RSC and freeze strategies, we propose discarding part of the accuracy scale gradients to improve the model's generalization performance.




Furthermore, through statistical analysis, we found that when the gradient disorder of the accuracy scale decreases to a certain level, the gradients in some layers enter a state of reverse balance. In other words, there is a significant overlap between the layers where reverse balance occurs and those where the accuracy scale’s disorder decreases. 



\textbf{Assumption 3.1} (The Impact of Incomplete Scale Convergence on Other Scales).
Observations show that some scales are able to reach a state of reverse balance between the accuracy scale (acc scale) and the smoothness scale (smooth scale), exhibiting signs of convergence. However, it is important to recognize that this apparent convergence does not necessarily mean that either the acc scale or the smooth scale has achieved satisfactory convergence. Further observations reveal that the layers with gradually decreasing gradient disorder in the acc scale highly coincide with those that ultimately reach this state of reverse balance convergence. This improper convergence could adversely affect the training of the smoothness scale and may not only affect the training effectiveness of specific layers but could also impact the training of other layers, including the emergence of outlier gradients.

To verify this hypothesis, we conducted an experiment. We used the gradient disorder of the accuracy scale as an indicator of convergence. Figure \ref{fig:freeze1}
\begin{figure}[htbp]
    \centering
    % First image
    \begin{minipage}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{freeze1.png}
        \caption{Enter Caption for Freeze 1}
        \label{fig:freeze1}
    \end{minipage}
    \hfill % Add some horizontal spacing
    % Second image
    \begin{minipage}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{freeze2.png}
        \caption{Enter Caption for Freeze 2}
        \label{fig:freeze2}
    \end{minipage}
\end{figure}

displays the gradient fluctuations of other scales after the accuracy scale has been frozen. The results demonstrate that not only does the frozen scale continue its smoothness training, but the gradient fluctuations in the unfrozen layers are significantly reduced. This finding underscores that the smoothness scale gradients have not achieved optimal convergence, and the suboptimal convergence of one scale and the training interference among different scales can affect gradient stability.


% Based on this, we hypothesize that freezing the accuracy scale with low disorder can enhance the learning of the smoothness scale. To test this hypothesis, we conducted a simple experiment. Figure x shows the real gradient changes of the same scale under frozen and unfrozen accuracy scale conditions, while Figure x2 shows the gradient changes of other scales after freezing the accuracy scale in Figure x. The results indicate that the frozen scale continues smoothness training, while the gradient fluctuations of other unfrozen layers are significantly reduced. This suggests that the instability in gradient fluctuations is partly caused by interference between scales during training.




We conclude that selectively freezing the accuracy scale can effectively solve the issue of scale instability during training and improve the insufficient convergence of the smoothness scale. However, continuously freezing the accuracy scale without unfreezing it could lead to suboptimal training results. Therefore, we adopt a dynamic strategy: every K steps, we assess the disorder. If the disorder is below a threshold \( r \), we freeze the scale for K steps; otherwise, we unfreeze it. Every K steps, we reselect the freezing range. We summarize our method in Algorithm \ref{alg:freeze}. 
\begin{algorithm}
\caption{Dynamic Selective Freezing Strategy for Multiple Scales}
\begin{algorithmic}[1]
\label{alg:freeze}
\State \textbf{Input:} Training steps $K$, threshold $r$, set of scales $\{S_1, S_2, \dots, S_n\}$
\State \textbf{Initialize:} $t = 0$ (step counter), $freeze[S_i] = False$ for all scales $S_i$
\While {training not finished}
    \For{each scale $S_i$}
        \If {$freeze[S_i] == True$}
            \State Freeze $S_i$ accuracy scale gradient 
        \Else
            \State Continue use both accuracy and smoothness scale gradients for $S_i$
        \EndIf
    \EndFor
    \If {every $K$ steps}
        \State Calculate accuracy gradient disorder $\delta_{t, S_i}$ for scale $S_i$ at step $t$
        \If {$\delta_{t, S_i} < r$}
            \State $freeze[S_i] \gets True$
        \Else
            \State $freeze[S_i] \gets False$
        \EndIf
    \EndIf
    \State $t \gets t + 1$ \Comment{Increment step counter}
\EndWhile
\end{algorithmic}
\end{algorithm}




% % 可能对smooth产生影响，次优







% % OB1 3.2 准确率scale梯度混乱度的逐渐减弱

% % 选择性冻结调度策略
% % 解释，伪代码



% % 实验结果  冻结old之后的平衡性质
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{image.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}
% %我们定义梯度的混乱度为每n步里面第k步和第k-1步梯度方向相反的梯度占n个梯度的比例，混乱度越低则说明当前梯度的学习方向较为统一，而混乱都越高则说明梯度具有一定的不确定性。同样在pacs数据集上，我们用art域作为测试集，其他域作为训练集，我们对准确率scale和平滑scale分别进行了测量，同样是每300步我们记录了这300步所有的梯度，图x表示了第102个scale的准确率梯度和平滑性梯度混乱度随训练的变化情况，我们发现部分层会出现准确率梯度的混乱度随着训练进行逐渐变低，也就是越发一致，而平滑梯度则在所有的层中都表现出较大且不随训练进行明显变化的混乱度。这启发我们部分层的准确率scale收敛可能会显著影响平滑scale的收敛。
% We define "gradient disorder" as the proportion of gradients in n steps where the direction of the gradient at step k is opposite to that at step k-1, relative to the total number of gradients in those n steps. A lower disorder indicates that the gradient learning direction is more consistent, while a higher disorder suggests greater uncertainty in the gradient directions.

% In experiments on the PACS dataset, we used the art domain as the test set and the other domains as the training set. We measured the accuracy scaling factor and smoothness scaling factor, recording all gradients every 300 steps and calculating their disorder. Figure x shows the changes in the disorder of the accuracy gradient and smoothness gradient of the 102nd scaling factor during training. We observed that, for some layers, the disorder of the accuracy gradients gradually decreases as training progresses, indicating more consistent gradient directions. However, the smoothness gradients exhibited consistently high disorder across all layers, with no significant change during training.

% This finding suggests that the convergence of the accuracy scaling factor in certain layers may significantly influence the convergence of the smoothness scaling factor.
% \subsection{准确率scale和平滑scale的平衡性}
% %同样有意思的一个观测是随着训练的进行，在部分层会出现一个准确率scale和平滑scale的梯度反向并且接近平衡的一个状态，也就是说这些层的scale会进入一个收敛的状态, 但是很显然，就单个准确率scale或者平坦性scale而言，这些层都未收敛，也就是说在准确性和平坦性上，这些层的scale其实进行了一个平衡，更有意思的是，同观测2的实验设置下，我们发现往往是最后准确率scale混乱度低的scale收敛平衡的更快更早，这启发我们或许是准确率scale混乱度低的scale的平滑性学习不足。
% Another interesting observation is that, as training progresses, the gradients of the accuracy scaling factor and the smoothness scaling factor in some layers gradually reverse and approach a balanced state, indicating that the scaling factors in these layers reach a certain convergence. However, when looking at the accuracy or smoothness scaling factors individually, these layers have not fully converged; rather, they achieve a balance between accuracy and smoothness.

% More intriguingly, in the same experimental setup as Observation 2, we found that the scaling factors with lower gradient disorder in the accuracy scaling factor tend to reach this balanced convergence state faster and earlier. This suggests that the scaling factors with lower accuracy gradient disorder may have insufficient smoothness learning.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{image.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}
% \subsection{冻结减小梯度冲突}
% %对于增强平滑性的学习，并且减弱梯度的异常跳变程度，我们尝试在某个scale达到平衡之后冻结某一层的准确率scale，只采纳平滑scale。如图x所示，这表示同一个scale在冻结准确率scale和未冻结两种情况下的真实梯度和情况，图x2表示在冻结了图1的准确率scale之后以及未冻结的情况下其余scale的梯度情况，可以发现被冻结的scale会开始继续训练，也就是平滑性会继续训练，而其他未冻结层的梯度波动程度显著减小。这启发我们可以采取选择性冻结的方式来优化训练过程中的scale不稳定性以及平滑性收敛不足的问题。
% To enhance smoothness learning and reduce abnormal gradient jumps, we attempted to freeze the accuracy scaling factor of a layer once a certain scaling factor (scale) reached equilibrium, while continuing to update only the smoothness scaling factor. As shown in Figure x, the gradient changes in the frozen and unfrozen accuracy scaling factor states are displayed. Figure x2 shows the gradient changes of other layers after freezing the accuracy scaling factor from Figure x. The results indicate that the frozen scaling factor continues smoothness training, and the gradient fluctuations in other unfrozen layers are significantly reduced. This finding suggests that selective freezing of accuracy scaling factors can effectively reduce instability in scaling factors during training and improve insufficient convergence in smoothness.
% 基于上面的观测，我们提出了一种在DG场景下适用的选择性冻结量化策略，它采用梯度的混乱度作为判断冻结的标准，在训练过程中不断的冻结满足标准的准确率scale的梯度，在不满足标准时解冻，选择性解耦优化部分层的scale训练，旨在减弱准确率scale和平坦性scale之间的梯度冲突，显著提升了scale的训练稳定性以及导向更优的泛化性。

% 跟踪梯度的抖动程度成了我们的重点

% \subsection{Footnotes}

% Indicate footnotes with a number\footnote{Sample of the first footnote} in the
% text. Place the footnotes at the bottom of the page on which they appear.
% Precede the footnote with a horizontal rule of 2~inches
% (12~picas).\footnote{Sample of the second footnote}

% \subsection{Figures}

% All artwork must be neat, clean, and legible. Lines should be dark
% enough for purposes of reproduction; art work should not be
% hand-drawn. The figure number and caption always appear after the
% figure. Place one line space before the figure caption, and one line
% space after the figure. The figure caption is lower case (except for
% first word and proper nouns); figures are numbered consecutively.

% Make sure the figure caption does not get separated from the figure.
% Leave sufficient space to avoid splitting the figure and figure caption.

% You may use color figures.
% However, it is best for the
% figure captions and the paper body to make sense if the paper is printed
% either in black/white or in color.
% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% \end{center}
% \caption{Sample figure caption.}
% \end{figure}

% \subsection{Tables}

% All tables must be centered, neat, clean and legible. Do not use hand-drawn
% tables. The table number and title always appear before the table. See
% Table~\ref{sample-table}.

% Place one line space before the table title, one line space after the table
% title, and one line space after the table. The table title must be lower case
% (except for first word and proper nouns); tables are numbered consecutively.

% \begin{table}[t]
% \caption{Sample table title}
% \label{sample-table}
% \begin{center}
% \begin{tabular}{ll}
% \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
% \\ \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
% \end{tabular}
% \end{center}
% \end{table}
